Block-Recurrent Transformers

We introduce the Block-Recurrent Transformer, which applies a transformer layer in a recurrent fashion along a sequence, and has linear complexity with respect to sequence length. Our recurrent cell operates on blocks of tokens rather than single tokens during training, and leverages parallel computation within a block in order to make efficient use of accelerator hardware. The cell itself is strikingly simple. It is merely a transformer layer: it uses self-attention and cross-attention to efficiently compute a recurrent function over a large set of state vectors and tokens. Our design was inspired in part by LSTM cells, and it uses LSTM-style gates, but it scales the typical LSTM cell up by several orders of magnitude. Our implementation of recurrence has the same cost in both computation time and parameter count as a conventional transformer layer, but offers dramatically improved perplexity in language modeling tasks over very long sequences. Our model out-performs a long-range Transformer XL baseline by a wide margin, while running twice as fast. We demonstrate its effectiveness on PG19 (books), arXiv papers, and GitHub source code. Our code has been released as open source.

==> sections/checklist.tex <==

\section{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work? \\
    \answerYes{See Section \ref{section:ethics}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \\
    \answerYes{We plan to open-source the code itself, although we have not yet done so.  We have given a detailed description of architecture, hyper-parameters, and training methodology.  Our main results are for PG19, which is a publicly available dataset.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{appendix:training-details}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \\
    \answerYes{Given the large number of experiments, we did not have the computational resources to run every experiment multiple times, but we do run experiments over multiple datasets. For the main headline numbers on PG19-tokens, we ran the primary experiments three times each with different initial seeds and with dataset shuffling.  Error bars are given in Table \ref{table:results}.  Note that actual measured error bars are somewhat lower than reported in Table \ref{table:results}; we round results to the nearest 0.01, and thus round the error \emph{up} to match the precision of the reported results.  See Appendix \ref{appendix:training-details}
    for details.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{appendix:training-details}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix \ref{appendix:dataset-license}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Appendix \ref{appendix:dataset-license}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix \ref{appendix:dataset-license}.}
\end{enumerate}

\end{enumerate}
